Give Me Some Slack: Efficient Network Measurements

Many networking applications require timely access to recent network measurements, which can be captured using a sliding window model. Maintaining such measurements is a challenging task due to the fast line speed and scarcity of fast memory in routers. In this work, we study the impact of allowing \emph{slack} in the window size on the asymptotic requirements of sliding window problems. That is, the algorithm can dynamically adjust the window size between $W$ and $W(1+\tau)$ where $\tau$ is a small positive parameter. We demonstrate this model's attractiveness by showing that it enables efficient algorithms to problems such as MAX and GENERAL-SUM that require $\Omega(W)$ bits even for constant factor approximations in the exact sliding window model. Additionally, for problems that admit sub-linear approximation algorithms such as BASIC-SUMMING and COUNT-DISTINCT, the slack model enables a further asymptotic improvement.

==> logw_lb.tex <==
\begin{lemma}\label{lem:logw}
	Let $\eps\le1/4$. Any deterministic algorithm that solves the \ADDI{} problem must use at least $\floor{\log W}$ bits.
\end{lemma}
\begin{proof}
%Note that $W$ is an integer and thus $\log W-1<\floor{\log W}$.
Assume by contradiction that \alg{} solves the \ADDI{} problem while using at most $m\triangleq \floor{\log W - 1}$ bits.
Consider \alg{}'s run on the input $0^{W(1+\tau)}R^{W(1+\tau)}$; i.e., the input consists of $W(1+\tau)$ zeros and then $W(1+\tau)$ times $R$. 
Consider the prefix set $P\triangleq \set{0^{W(1+\tau)}R^{i}\mid i\in[\floor{W/2}]}$. 
Since $|P|=\floor{W/2}+1 > 2^m$, there has to be two distinct prefixes $p_1\subsetneq p_2\in P$ such that \alg{}'s run on $p_1$ reaches the same memory configuration $\mathfrak{c}$ as it would reach running on $p_2$.  
We denote the number of $R$'s in $p_1$ and $p_2$ by $r_1$ and $r_2$, respectively. 
Being a deterministic algorithm, \alg{} must return to $\mathfrak{c}$ after processing the input $0^{W(1+\tau)}R^{r_1}R^{z\cdot(r_2-r_1)}$, for any integer $z$. 
Specifically, it must reach this configuration after seeing $p_3\triangleq0^{W(1+\tau)}R^{r_1}R^{W(1+\tau)\cdot(r_2-r_1)}$, so that the last $W(1+\tau)$ elements are all $R$. 
As a deterministic algorithm, the output of \alg{} at configuration $\mathfrak{c}$, $\langle\widehat{S},c\rangle$ is fixed, and should approximate the sum after seeing \emph{any} input sequence that leads it to $\mathfrak{c}$. 
Thus, the algorithm's answer must satisfy:
\begin{enumerate}
\item $\widehat{S} \le R\cdot r_1 +\bserror < R\cdot\floor{W/2} + \bserror$ \hfill (answering for $p_1$)
\item $\widehat{S} \ge R\cdot W -\bserror$ \hfill (answering for $p_3$)
\end{enumerate}
But these two cannot exist together as $\eps\le1/4$. A contradiction.
\end{proof} 


==> preamble.tex <==

%This is a template for producing LIPIcs articles.
%See lipics-manual.pdf for further information.
%for A4 paper format use option "a4paper", for US-letter use option "letterpaper"
%for british hyphenation rules use option "UKenglish", for american hyphenation rules use option "USenglish"
% for section-numbered lemmas etc., use "numberwithinsect"

%\usepackage{microtype}%if unwanted, comment out or use option "draft"

\input{macros.tex}

%\graphicspath{{./graphics/}}%helpful if your graphic files are in another directory

\bibliographystyle{plain}% the recommended bibstyle

% Author macros::begin %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{comment}
%\usepackage{fullpage}
%\usepackage[british]{babel}
\usepackage{url}
%\usepackage{dsfont}
%\let\proof\relax
%\let\endproof\relax
\usepackage{amsmath,amssymb}
\usepackage{float}
\usepackage{multirow}% http://ctan.org/pkg/multirow
\usepackage{hhline}% http://ctan.org/pkg/hhline
\usepackage{calc}
\usepackage{amsthm}
%\usepackage{dstroke}
%\usepackage{breqn}
%\usepackage[]{algorithm2e}

\usepackage{graphicx}
\usepackage{framed}
\usepackage{xspace}
\usepackage{algorithm}
%\usepackage[hang]{subfigure}
\usepackage[noend]{algpseudocode}
\usepackage{algorithm}
\usepackage{array}


\newtheorem{thm}{Theorem}[section] % the main one
%\newtheorem{lemma}[thm]{Lemma}

\swapnumbers

\theoremstyle{plain} % just in case the style had changed
\newcommand{\thistheoremname}{}
\newtheorem{genericthm}[thm]{\thistheoremname}
\newenvironment{namedprb}[1]
  {\renewcommand{\thistheoremname}{#1}%
   \begin{genericthm}}
  {\end{genericthm}}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}


%\newenvironment{definition}[1][Definition]{\begin{trivlist}
% 		\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{example}[1][Example]{\begin{trivlist}
%% 		\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{remark}[1][Remark]{\begin{trivlist}
% 		\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}


\renewcommand{\qed}{\nobreak \ifvmode \relax \else
	\ifdim\lastskip<1.5em \hskip-\lastskip
	\hskip1.5em plus0em minus0.5em \fi \nobreak
	\vrule height0.75em width0.5em depth0.25em\fi}

\providecommand{\tabularnewline}{\\}
\newtheorem{obs}{Observation}

\newcommand{\omn}[1]{ {\{0,1\}^{#1}} }
\def\half{ \frac{1}{2}}
\newcommand{\ip}[2]{\langle #1,#2 \rangle}
\def\sumN{\sum_{i=1}^n}
\def\_{\,\,\,\,\,}
\def\prob{{\mathbf{Pr}}}

\newcommand{\Hi}{ {\mbox{H}_{\infty}} }
\newcommand{\w}{w}
\def\modulo{\text{mod}}

\def\D{{\partial}}
\def\gap{\text{gap}}
\def\sign{\text{sign}}
\def\sing{\text{Sing}}
\def\rank{\text{rank}}
\def\cp{\text{cp}}

\newcommand{\jac}[2]{$\frac{\D #1}{\D #2}$}
\newcommand{\jacm}[2]{\frac{\D #1}{\D #2}}
\newcommand{\leftar}{\leftarrow}
\newcommand{\B}{\{0,1\}}
\newcommand{\ar}{\rightarrow}

\newcommand{\anote}[1]{{\bf Ariel's note: \{}{\sf#1}{\bf\}}}



%macros for this paper;

\def\kofr{L_k^{V_1,\ldots,V_r}}
\def\kofrsimp{L_{k-simp}^{V_1,\ldots,V_r}}
\def\kdistinct{L_k}
\def\simpk{\textrm SIMPLE $\mathrm{k}$-PATH\xspace}
\def\stsimpk{{\textrm SIMPLE $\mathrm{(s,t)}$-$\mathrm{k}$-PATH }\xspace}
\def\minwt{{\textrm MIN-WT SIMPLE $\mathrm{k}$-PATH}\xspace}
\def\stminwt{{\textrm MIN-WT SIMPLE $\mathrm{(s,t)}$-$\mathrm{k}$-PATH}\xspace}
\def\ktsp{$\mathrm{k}$ \textrm{-TSP}\xspace}
\def\kstroll{$\mathrm{k}$-\textrm{STROLL}\xspace}
\def\ktour{$\mathrm{k}$-\textrm{TOUR}\xspace}

\def\kpath{{$\mathrm{k}$-path}\xspace}
\def\stpath{$\mathrm{(s,t)}$-\textrm{path}\xspace}
\def\stkpath{$\mathrm{(s,t)}$-$\mathrm{k}$-path\xspace}

\newcommand{\Var}{\mathrm{Var}}
\newcommand{\cov}{\mathrm{cov}}
\def\poly{n^{O(1)}}
\newcommand{\polylog}{\mbox{\mathrm{polylog}}}
\newcommand{\xorL}{ L_{\oplus}}
\newcommand{\F}{{\mathbb F}}

\newcommand{\zeros}[1]{\mathrm{ZEROS}_{>#1}}
\newcommand{\prev}{\mathrm{prev}}
%\newcommand{\next}{\mathrm{next}}
\newcommand{\size}{\mathrm{size}}


\newcommand{\epsclose}{\stackrel{\epsilon}{\thicksim} }
 \newcommand{\eclose}[1]{\stackrel{{#1}}{\thicksim} }
 \def\Pr{{\mathrm{Pr}}}
 \def\pr{{\mathrm{Pr}}}
\newcommand{\power}[1]{2^{#1}}
\def\Supp{{\mathrm{Supp}}}
\def\supp{{\mathrm{Supp}}}
\def\E{{\mathrm{E}}}
\def\R{{\mathbb{R}}}
\newcommand{\M}{{\cal M}}
\newcommand{\N}{{\cal N}}
\newcommand{\A}{{\cal A}}
\newcommand{\Cd}{{\cal C}}
\newcommand{\rate}{\mbox{rate}}
\newcommand{\rparagraph}[1]{\vspace{-0.15in} \paragraph{#1}}
%\newcommand{\rparagraph}[1]{\paragraph{#1}}
\newcommand{\ritem}{\vspace{-0.1in} \item}
%\newcommand{\ritem}{\item}
\newcommand{\itab}[1]{\hspace{0em}\rlap{#1}}
\newcommand{\tab}[1]{\hspace{.12\textwidth}\rlap{#1}}
\newcommand{\htab}[1]{\hspace{.05\textwidth}\rlap{#1}}


%\newcommand{\rsubsection}[1]{\vspace{-0.1in} \subsection{#1} \vspace{-0.05in}}
\newcommand{\sett}[2]{\set{#1}_{#2}}

\newcommand{\negA}{}
\newcommand{\negB}{}
\newcommand{\negC}{}
\newcommand{\posA}{}
\newcommand{\mysection}[1]{\negC\section{#1}\negA}
\newcommand{\mysubsection}[1]{\negB\subsection{#1}\negA}
\newcommand{\mysubsubsection}[1]{\negB\subsubsection{#1}\negA}
\newcommand{\myparagraph}[1]{\par\smallskip\par\noindent{\bf{}#1:~}}

\newcommand{\rnote}[1]{{\bf Ran's note: \{}{\sf#1}{\bf\}}}

%\renewcommand{\algorithmicforall}{\textbf{for each}}

\usepackage[noend]{algpseudocode}
%\usepackage{enumitem}
%\setlist[description]{style=multiline,leftmargin=3.5cm, align=parright,noitemsep}
%\usepackage{enumitem}
%\SetLabelAlign{parright}{\strut\smash{\parbox[t]{\labelwidth}{\raggedleft#1}}}
\usepackage{multicol}
\usepackage{amsthm}
\usepackage{amsmath} 
